A Study on Robustness to Perturbations for Representations of Environmental Sound

Audio applications involving environmental sound analysis increasingly use general-purpose audio representations, also known as embeddings, for transfer learning. Recently, Holistic Evaluation of Audio Representations (HEAR) evaluated twenty-nine embedding models on nineteen diverse tasks. However, the evaluation's effectiveness depends on the variation already captured within a given dataset. Therefore, for a given data domain, it is unclear how the representations would be affected by the variations caused by myriad microphones' range and acoustic conditions -- commonly known as channel effects. We aim to extend HEAR to evaluate invariance to channel effects in this work. To accomplish this, we imitate channel effects by injecting perturbations to the audio signal and measure the shift in the new (perturbed) embeddings with three distance measures, making the evaluation domain-dependent but not task-dependent. Combined with the downstream performance, it helps us make a more informed prediction of how robust the embeddings are to the channel effects. We evaluate two embeddings -- YAMNet, and OpenL3 on monophonic (UrbanSound8K) and polyphonic (SONYC-UST) urban datasets. We show that one distance measure does not suffice in such task-independent evaluation. Although Fr\'echet Audio Distance (FAD) correlates with the trend of the performance drop in the downstream task most accurately, we show that we need to study FAD in conjunction with the other distances to get a clear understanding of the overall effect of the perturbation. In terms of the embedding performance, we find OpenL3 to be more robust than YAMNet, which aligns with the HEAR evaluation.

==> format_dump.tex <==
% % \section{Ease of Use}

% % \subsection{Maintaining the Integrity of the Specifications}

% % The IEEEtran class file is used to format your paper and style the text. All margins, 
% % column widths, line spaces, and text fonts are prescribed; please do not 
% % alter them. You may note peculiarities. For example, the head margin
% % measures proportionately more than is customary. This measurement 
% % and others are deliberate, using specifications that anticipate your paper 
% % as one part of the entire proceedings, and not as an independent document. 
% % Please do not revise any of the current designations.

% % \section{Prepare Your Paper Before Styling}
% % Before you begin to format your paper, first write and save the content as a 
% % separate text file. Complete all content and organizational editing before 
% % formatting. Please note sections \ref{AA}--\ref{SCM} below for more information on 
% % proofreading, spelling and grammar.

% % Keep your text and graphic files separate until after the text has been 
% % formatted and styled. Do not number text heads---{\LaTeX} will do that 
% % for you.

% % \subsection{Abbreviations and Acronyms}\label{AA}
% % Define abbreviations and acronyms the first time they are used in the text, 
% % even after they have been defined in the abstract. Abbreviations such as 
% % IEEE, SI, MKS, CGS, ac, dc, and rms do not have to be defined. Do not use 
% % abbreviations in the title or heads unless they are unavoidable.

% % \subsection{Units}
% % \begin{itemize}
% % \item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
% % \item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
% % \item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
% % \item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
% % \end{itemize}

% % \subsection{Equations}
% % Number equations consecutively. To make your 
% % equations more compact, you may use the solidus (~/~), the exp function, or 
% % appropriate exponents. Italicize Roman symbols for quantities and variables, 
% % but not Greek symbols. Use a long dash rather than a hyphen for a minus 
% % sign. Punctuate equations with commas or periods when they are part of a 
% % sentence, as in:
% % \begin{equation}
% % a+b=\gamma\label{eq}
% % \end{equation}

% % Be sure that the 
% % symbols in your equation have been defined before or immediately following 
% % the equation. Use ``\eqref{eq}'', not ``Eq.~\eqref{eq}'' or ``equation \eqref{eq}'', except at 
% % the beginning of a sentence: ``Equation \eqref{eq} is . . .''

% % \subsection{\LaTeX-Specific Advice}

% % Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
% % of ``hard'' references (e.g., \verb|(1)|). That will make it possible
% % to combine sections, add equations, or change the order of figures or
% % citations without having to go through the file line by line.

% % Please don't use the \verb|{eqnarray}| equation environment. Use
% % \verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
% % environment leaves unsightly spaces around relation symbols.

% % Please note that the \verb|{subequations}| environment in {\LaTeX}
% % will increment the main equation counter even when there are no
% % equation numbers displayed. If you forget that, you might write an
% % article in which the equation numbers skip from (17) to (20), causing
% % the copy editors to wonder if you've discovered a new method of
% % counting.

% % {\BibTeX} does not work by magic. It doesn't get the bibliographic
% % data from thin air but from .bib files. If you use {\BibTeX} to produce a
% % bibliography you must send the .bib files. 

% % {\LaTeX} can't read your mind. If you assign the same label to a
% % subsubsection and a table, you might find that Table I has been cross
% % referenced as Table IV-B3. 

% % {\LaTeX} does not have precognitive abilities. If you put a
% % \verb|\label| command before the command that updates the counter it's
% % supposed to be using, the label will pick up the last counter to be
% % cross referenced instead. In particular, a \verb|\label| command
% % should not go before the caption of a figure or a table.

% % Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
% % will not stop equation numbers inside \verb|{array}| (there won't be
% % any anyway) and it might stop a wanted equation number in the
% % surrounding equation.

% % \subsection{Some Common Mistakes}\label{SCM}
% % \begin{itemize}
% % \item The word ``data'' is plural, not singular.
% % \item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
% % \item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
% % \item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
% % \item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
% % \item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
% % \item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
% % \item Do not confuse ``imply'' and ``infer''.
% % \item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
% % \item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
% % \item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
% % \end{itemize}
% % An excellent style manual for science writers is \cite{b7}.

% % \subsection{Authors and Affiliations}
% % \textbf{The class file is designed for, but not limited to, six authors.} A 
% % minimum of one author is required for all conference articles. Author names 
% % should be listed starting from left to right and then moving down to the 
% % next line. This is the author sequence that will be used in future citations 
% % and by indexing services. Names should not be listed in columns nor group by 
% % affiliation. Please keep your affiliations as succinct as possible (for 
% % example, do not differentiate among departments of the same organization).

% % \subsection{Identify the Headings}
% % Headings, or heads, are organizational devices that guide the reader through 
% % your paper. There are two types: component heads and text heads.

% % Component heads identify the different components of your paper and are not 
% % topically subordinate to each other. Examples include Acknowledgments and 
% % References and, for these, the correct style to use is ``Heading 5''. Use 
% % ``figure caption'' for your Figure captions, and ``table head'' for your 
% % table title. Run-in heads, such as ``Abstract'', will require you to apply a 
% % style (in this case, italic) in addition to the style provided by the drop 
% % down menu to differentiate the head from the text.

% % Text heads organize the topics on a relational, hierarchical basis. For 
% % example, the paper title is the primary text head because all subsequent 
% % material relates and elaborates on this one topic. If there are two or more 
% % sub-topics, the next level head (uppercase Roman numerals) should be used 
% % and, conversely, if there are not at least two sub-topics, then no subheads 
% % should be introduced.

% % \subsection{Figures and Tables}
% % \paragraph{Positioning Figures and Tables} Place figures and tables at the top and 
% % bottom of columns. Avoid placing them in the middle of columns. Large 
% % figures and tables may span across both columns. Figure captions should be 
% % below the figures; table heads should appear above the tables. Insert 
% % figures and tables after they are cited in the text. Use the abbreviation 
% % ``Fig.~\ref{fig}'', even at the beginning of a sentence.

% % \begin{table}[htbp]
% % \caption{Table Type Styles}
% % \begin{center}
% % \begin{tabular}{|c|c|c|c|}
% % \hline
% % \textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
% % \cline{2-4} 
% % \textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
% % \hline
% % copy& More table copy$^{\mathrm{a}}$& &  \\
% % \hline
% % \multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
% % \end{tabular}
% % \label{tab1}
% % \end{center}
% % \end{table}

% % \begin{figure}[htbp]
% % \centerline{\includegraphics{fig1.png}}
% % \caption{Example of a figure caption.}
% % \label{fig}
% % \end{figure}

% % Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
% % rather than symbols or abbreviations when writing Figure axis labels to 
% % avoid confusing the reader. As an example, write the quantity 
% % ``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
% % units in the label, present them within parentheses. Do not label axes only 
% % with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
% % \{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
% % quantities and units. For example, write ``Temperature (K)'', not 
% % ``Temperature/K''.

% % \section*{Acknowledgment}

% % The preferred spelling of the word ``acknowledgment'' in America is without 
% % an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
% % G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
% % acknowledgments in the unnumbered footnote on the first page.

% % \section*{References}

% % Please number citations consecutively within brackets \cite{b1}. The 
% % sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
% % number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
% % the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

% % Number footnotes separately in superscripts. Place the actual footnote at 
% % the bottom of the column in which it was cited. Do not put footnotes in the 
% % abstract or reference list. Use letters for table footnotes.

% % Unless there are six authors or more give all authors' names; do not use 
% % ``et al.''. Papers that have not been published, even if they have been 
% % submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
% % that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
% % Capitalize only the first word in a paper title, except for proper nouns and 
% % element symbols.

% % For papers published in translation journals, please give the English 
% % citation first, followed by the original foreign-language citation \cite{b6}.

% \begin{thebibliography}{00}
% \bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
% \bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
% \bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
% \bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
% \bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
% \bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
% \bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
% \end{thebibliography}
% \vspace{12pt}
% \color{red}
% IEEE conference templates contain guidance text for composing and formatting conference papers. Please ensure that all template text is removed from your conference paper prior to submission to the conference. Failure to remove the template text from your paper may result in your paper not being published.

==> misc.tex <==
% Juan's comments
- Magda/Mark? Recast the paper as a follow up to hear results (and discuss them in more detail in the intro). Relate the choice of embeddings and datasets with HEAR?

- Focus on the embedding displacement measures: CD and FAD and try to figure out the relationship between displacement and classification performance. 

- Sangeeta: I would strongly suggest to run classification on the perturbed samples.

- Sangeeta: I would suggest eliminating figures 2 and 5, modifying figure 1 s.t. it fits both CD and fad, and blowing figure 3 into a larger figure with more subplots that shows CD and fad separately.

- I am unsure about figure 4 and the topology measure altogether? 
Sangeeta - let's decide this later







% For 2/17 discussion
% - How to define the metric in Topology? It's not CPCC.
- How to leverage FSD datasets in a bare minimum sense?
- Discuss the plots we have and what we can say with those.
- Are we ready to conclude something specific about when which metric should be used?


% Mag + Sangeeta
2/14
- CPCC or CPCC Distance, i.e. 1-CPCC

Observations to discuss with Mag
- Comparison of representation
    - Openl3 does best (shows min variation) in CD and does worst in FAD whereas YamNet does best in FAD and does worst in CPCC. Actually, I do not know if a flatter curve in CD for Openl3 is a good thing or a bad thing. The fact that other metrics change show that the distributions do change so CD is misleading or FAD is misleading as it shows lot of variation even for a small perturbation? Maybe, we can say it is a good metric to test if things have changed even slightly but should not be used to test robustness? 
- Comparison of metrics
    - Sensitivity to dataset (FAD changes a lot from one dataset to another)
    - Sensitivity to batches (CPCC is most sensitive to subset selected for metric evaluation)
    - Sensitivity to perturbation

Dependency
- Get the index of the embedding that has highest SPL UST + US8K (Needed for Class Sensitivity)
- Get alpha for OpenL3 and redo the cosine distances


% Anish + Sangeeta
Across all perturbations and across all metrics (modified FAD), YAMNet is worse.

- Why do we need mean-shift (translation) in Eq. 4? The downstream classifier should be able to compensate for a translation effect.
- (Fig 4) Stick to green color for FAD. Also plot FAD without mean-shift.
- (Fig 4) OpenL3 shows a shift in the mean because it is sampling at a higher frequency (gotten rid of relatively more frequency components). This is why in US8K OpenL3 FAD is worse than YAMNet FAD. Variance shift in OpenL3 is not as large as YAMNet (coming from the formula of FAD).
- (Fig 4) Why is variance in YAMNet is 10x higher in UST?

Metrics
- Background: Mean cosine distance might cancel out the effects in case of noise (clutter). While CPCD might be a better choice for such cases, it is sensitive to subset selection and so should be used with enough diversity and coverage.
- @Mark: Lot of frontend variations -> phase distortions. This might affect CD. 

==> old_intro.tex <==
Scarcity of large amount of labeled data for supervised learning in applications related to environmental sounds has popularized the use of representation learning and transfer learning \cite{cramer2019look, jansen2020coincidence, wang2021multi, alayrac2020self}. As part of this learning paradigm, a network is pre-trained on an \textit{upstream} task which has availability of large datasets to learn generic representations or embeddings that can be used to transfer-learn classifier(s) on a variety of related target \textit{downstream} application(s). Having access to such vast amounts of upstream data \cite{gemmeke2017audio} allows pre-trained models to be over-parameterized, which has been shown to be the an essential element in attaining generalization \cite{brutzkus2019larger}. 
This has been shown to be true for audio classification scenarios \cite{cramer2019look}, and the hope is that the learnt representations are more robust and therefore not sensitive to small changes, also called \textit{perturbations} in the audio signal.

Recent works have addressed robustness by
assessing the embeddings' classification performance in a downstream task(s) \cite{grollmisch2021analyzing}. This has been popularized by recent challenges and benchmarks, organized first within the computer vision community \cite{goyal2019scaling}, and more recently in the machine listening community, e.g. Holistic Audio Representation Evaluation Suite (HARES) \cite{wang2021towards}, Holistic Evaluation of Audio Representations (HEAR) \cite{turian2022hear}. The HEAR challenge is the largest effort to date to evaluate audio representations. Several embeddings were submitted and ranked across different downstream tasks including music, speech and environmental sound.

These approaches, while valuable, do not provide information regarding the stability of such embeddings in response to specific changes in the data, and hence do not aid in understanding what to expect when employing them in real-world applications under various conditions. Furthermore, using labeled data to assess embedding has the inherent drawback of requiring human annotations, making it difficult to scale to multiple contexts and applications. While researchers have attempted to circumvent the data limitation by artificially degrading audio signals \cite{de2021analysis, serizel2020sound} with tools such as ADT \cite{mauch2013audio} or Scaper \cite{salamon2017scaper}, the robustness analysis remains ``solely" dependent on the end application.

In the deep learning community, approaches to robustness are often performed by applying different mathematical transformations or \textit{perturbations} to the input of a deep learning model, and theoretically assessing its impact on the output, followed by experimental validation \cite{bietti2017invariance, bietti2019group}. The advantage of these approaches is that they are task-agnostic and thus have the potential to generalize to a larger umbrella of applications. Our evaluation pipeline is inspired by these methods. In this paper, we propose to use distance metrics to compare the shift solely in the embedding space, making the evaluation methodology task-free. We further correlate the metrics with the downstream results to corroborate the findings and establish relationship between the perturbations and the downstream evaluation. We leverage two publicly available audio embedding models, \textit{OpenL$^3$} \cite{cramer2019look} and \textit{YAMNet\footnote{https://github.com/tensorflow/models/tree/master/research/audioset/yamnet}}, to build on the findings from the HEAR challenge, where OpenL$^3$ and YAMNet were reported to be among the best and worst performing models, respectively.

Our contributions can be summarized as follows:
1) We propose a principled methodology to evaluate robustness of audio embeddings against channel effects, both qualitatively and quantitatively, in a task-free setting. 
2) We investigate the use and limitations of three distance measures for analyzing changes in pairwise distance, topology, and distribution in order to gain insight into downstream performance.
3) We mimic channel effects with four basic perturbations: high pass (HP) and low pass (LP) filtering, gain and reverberation and show gain and reverberation to be more robust to channel effects than both HP and LP.
4) We show YAMNet to be less robust than OpenL$^3$ against the four perturbations.

==> prev.tex <==
% Previous Fig 3

% \begin{figure*}[htb]
% \centering
% \subfloat{
%   \centering
%     \includegraphics[width=0.49\linewidth]{images/us8k.png}
% }
% \subfloat{
%   \centering
%     \includegraphics[width=0.49\linewidth]{images/ust.png}
% }
% \caption{CD, CPCD, and FAD for US8K and UST datasets for four perturbation types. The x-axis values for each perturbation range from a minor to a large change. The sampling frequency of YAMNet and OpenL$^3$ is 16kHz and 44.1kHz, respectively.}
% \label{fig:eval_metrics}
% \end{figure*}

% Discussion around FAD (Previous Fig 4)

\begin{figure}[htb]
% \centering
% \subfloat{
%   \centering
%     \includegraphics[width=0.245\linewidth]{images/yamnet_us8k.png}
%     \label{fig:y_us8k}
%     % \caption{}
% }
\subfloat{
  \centering
    \includegraphics[width=0.48\linewidth]{images/yamnet_ust.png}
    \label{fig:y_ust}
    % \caption{}
}
% \subfloat{
%   \centering
%     \includegraphics[width=0.2315\linewidth]{images/openl3_us8k.png}
%     \label{fig:o_us8k}
%     % \caption{}
% }
\subfloat{
  \centering
    \includegraphics[width=0.48\linewidth]{images/openl3_ust.png}
    \label{fig:o_ust}
    % \caption{}
}
\caption{FAD terms for embeddings of \textit{car-horn} and \textit{siren} class for low-pass perturbation in US8K and UST.}
\label{fig:siren}
\end{figure}

\noindent \textbf{CPCD}: For both US8K and UST, CPCD is higher for YAMNet than OpenL$^3$. \COMMENT{Based on the Fig. 2, we can say that CPCD is sensitive to noise. So, can we make the following conclusions? 1) YAMNet will be worse than OpenL3 for noisy (clutter/background) data? We get similar conclusion when we compare US8K and UST where the latter is a dataset with more background/clutter.
2) Gain beyond 10 dB introduces significant noise (maybe right thing to say is raises noise floor) and it affects both the embeddings.}

Furthermore, in high-pass and low-pass for US8K, the change in distance measures for OpenL$^3$ is more gradual than for YAMNet, resulting in a concave shape for the former and a convex shape for the latter. Overall, OpenL$^3$ is robust to changes in reverberation. \COMMENT{How to explain this?}

\noindent \textbf{FAD}: While OpenL$^3$ outperforms YAMNet in high-pass and low-pass for UST, the trend inverts in US8K, with the difference being most pronounced in low-pass. To better understand the trend difference in low-pass, we look at the distribution change in the \textit{siren} and \textit{car-horn} classes in both datasets for a fair comparison. We specifically look at the the three terms in Equation \ref{eq:fad} separately: a) shift in the mean ($\mu\_shift \! = \! ||\mu_o - \mu_p||_2^2$), b) variance in the original distribution ($o\_var \!= \!tr(\Sigma_o$), and c) variance in the perturbed distribution ($p\_var \!= \!tr(\Sigma_p$)). In Fig. \ref{fig:y_ust}, we observe that the variance of the perturbed YAMNet embeddings, $p\_var$, increases by more than 81$\times$ for cut-off frequencies beyond 1600 Hz, resulting in a large change in the FAD. Another important observation to make is the pattern in which the distributions for both the representations change. The mean for YAMNet does not change significantly as the cut-off frequency decreases for low-pass, but the embeddings get increasingly spread out, shown by the large $p\_var$. OpenL$^3$, on the other hand, has a bigger mean shift with minimized variance. The higher FAD for OpenL$^3$ in US8K is due to this larger shift in the mean as compared to YAMNet. \COMMENT{Should we say anything about the variance trend?}

% \subsection{Sensitivity of distance metrics to subset sampling}

% When there is a large number of audio snippets on which one wants to evaluate robustness, the distance matrix for CPCD and covariance matrices for FAD can be memory bottlenecks. So, it is natural to sample a subset of audio snippets for testing. We test the variation in the distance measures when different subsets are chosen for a given perturbation type and value. We divide the US8K dataset into batches of 128 data points and calculate the standard deviation among the resulting subsets. 
% In Fig. \ref{fig:batches}, we can see that CPCD is the most sensitive metric to subset selection and for even small perturbations, the distance values can have a high standard deviation ($stdev.$). YAMNet is in general more susceptible to change as compared to OpenL$^3$, with reverberation yielding the worst $stdev. > 0.25$. While we observe that both FAD and CPCD become sensitive when the perturbation is severe, the spread is significant for \textit{high-pass} and \textit{low-pass} in YAMNet. A similar trend is observed for UST dataset.

% \begin{figure}[htb]
%  \includegraphics[width=\linewidth]{images/batches.png}
% \caption{Standard deviation (stdev.) of metrics across different subsets of UrbanSound8K}
%     \label{fig:batches}
% \end{figure}

% \subsection{Case Study: Comparison of different datasets}
% \subsubsection{Multi-class vs. Multi-label}

% \subsection{Case Study: Class sensitivity to the perturbations}

% \section{Discussion}
% \COMMENT{Can we give insights on which metric is better in the following cases:
% \begin{enumerate}
%     \item Datasets with high background noise
%     \item Large acoustic datasets to be used for evaluation
%     \item Dataset with long-tailed distribution
%     \item Dataset with outliers
% \end{enumerate}
% }
% \COMMENT{Thought dump. If someone can help me write some conclusion here regarding the 3 metrics, that would be helpful.} Cosine distance is not so helpful and can lead to misleading conclusions \COMMENT{if not normalized properly w.r.t the original distance distribution}. Although FAD is most useful in detecting distribution shifts, when the use-case is to detect the effect on the separability of points or clustering, FAD does not give a direct conclusion and therefore, CPCD is a more preferable metric. Nevertheless, CPCD is sensitive to the sample size and distribution. When these three metrics are used, we recommend to sample a large (if not all) and diverse subset of data-points for CPCD and use that along with FAD to have a more accurate understanding of the effect of perturbation. \COMMENT{There are other metrics which might be more ..... which we leave for future work?}


\begin{figure*}[htb]
\centering
\subfloat{
  \centering
    \includegraphics[width=0.46\linewidth]{images/CD.png}
}
\subfloat{
  \centering
    \includegraphics[width=0.46\linewidth]{images/CPCD.png}
}
\caption{}
\label{fig:cd_cpcd}
\end{figure*}

\begin{figure*}[htb]
\centering
\subfloat{
  \centering
    \includegraphics[width=0.46\linewidth]{images/FAD.png}
}
\subfloat{
  \centering
    \includegraphics[width=0.46\linewidth]{images/US8K_accuracy.png}
}
\caption{}
\label{fig:fad}
\end{figure*}
